Black-box Safety Analysis and Retraining of DNNs based on Feature Extraction and Clustering

Deep neural networks (DNNs) have demonstrated superior performance over classical machine learning to support many features in safety-critical systems. Although DNNs are now widely used in such systems (e.g., self driving cars), there is limited progress regarding automated support for functional safety analysis in DNN-based systems. For example, the identification of root causes of errors, to enable both risk analysis and DNN retraining, remains an open problem. In this paper, we propose SAFE, a black-box approach to automatically characterize the root causes of DNN errors. SAFE relies on a transfer learning model pre-trained on ImageNet to extract the features from error-inducing images. It then applies a density-based clustering algorithm to detect arbitrary shaped clusters of images modeling plausible causes of error. Last, clusters are used to effectively retrain and improve the DNN. The black-box nature of SAFE is motivated by our objective not to require changes or even access to the DNN internals to facilitate adoption. Experimental results show the superior ability of SAFE in identifying different root causes of DNN errors based on case studies in the automotive domain. It also yields significant improvements in DNN accuracy after retraining, while saving significant execution time and memory when compared to alternatives.

==> algos/assignToClusters.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
%\begin{figure}[tb]

\begin{figure}

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
\Require (1) $R$, root cause clusters. (2) $DM_{TS}$, distance matrix for the unsafe test set \emph{TS} at layer L. The matrix is m x m, where m is the number of error-inducing inputs in TS. (3) $DM_{IS}$, distance matrix capturing the distance between images in the improvement set and images in \emph{TS}. (4) $U$, max number of improvement set images per cluster to return
\Ensure an associative array with the unsafe images associated to each root cause cluster
% (source inputs, follow-up inputs, output data).

%\Require $dm$, a domain model
%\Ensure $P$, a set of pairs $<Scenario, pc>$
%\State $step.visited = true$	
\State {$\mathit{unsafeImages} \gets \mathit{empty} \mathit{List}  $}; {$\mathit{unsafeSet} \gets \mathit{empty} \mathit{Set}  $}
\For{ y belonging to IS}
\For{ $C_{j}$ in R} \label{algo:unsafe:forC}
\State $\mathit{SSE}\_C_{j} = 0$; $\mathit{ICD}\_C_{j} = 0$ ; $\mathit{ICD}\_C_{j'} = 0$ ; $\mathit{pairs} = 0$
\For{ t, image belonging to $C_{j}$}
\For{ u, image belonging to $C_{j}$}
\If{index of t < index of u}
\State $\mathit{SSE}\_C_{j} \mathrel{+}= ( DM_{TS}[t][u] )^{2}$
\State $\mathit{ICD}\_C_{j} \mathrel{+}= DM_{TS}[t][u] $
\State $\mathit{pairs} \mathrel{+}= 1 $
\EndIf
\EndFor
\State $\mathit{SSE}\_C_{j'} \mathrel{+}= ( DM_{IS}[y][t] )^{2}$
\State $\mathit{ICD}\_C_{j'} \mathrel{+}= DM_{IS}[y][t]$
\EndFor % case of t
\State $\mathit{ICD}\_C_{j'} = ( \mathit{ICD}\_C_{j} + \mathit{ICD}\_C_{j'} ) / ( \mathit{pairs} + \mathit{sizeof}(C_j) )$
\State $\mathit{ICD}\_C_{j} = \mathit{ICD}\_C_{j} / \mathit{pairs}$
\State $\mathit{SSE}\_C_{j'} = ( \mathit{SSE}\_C_{j} + \mathit{SSE}\_C_{j'} ) / (\mathit{sizeof}(C_j)+1)$
\State $\mathit{SSE}\_C_{j} = \mathit{SSE}\_C_{j} / \mathit{sizeof}(C_j)$
\State $\mathit{store} ( y, c, \mathit{ICD}\_C_{j}, \mathit{ICD}\_C_{j'}, \mathit{SSE}\_C_{j}, \mathit{SSE}\_C_{j'} )$
\EndFor \label{algo:unsafe:distCompEnd}

\State { \emph{identify cluster} $\mathit{C_j}$ \emph{with minimal} $\mathit{SSE}\_C_{j'}$ \emph{and retrieve} $\mathit{ICD}\_C_{j'}$ \emph{and} $\mathit{ICD}\_C_{j}$ }

\If{$\mathit{ICD}\_C_{j'} \leq \mathit{ICD}\_C_{j}$} \label{algo:unsafe:check}
\State {$\mathit{unsafeImages} \gets \langle y, \mathit{C_j} \rangle$}
\EndIf
\EndFor 

\For{ $C_j$ in C}
\State {$\mathit{imgs} \gets$ \emph{select} $U$ \emph{images in} $\mathit{unsafeImages}$ \emph{with} lowest $\mathit{SSE\_C_{j'}}$ \emph{and} $C_j$ \emph{as right term}} \label{algo:unsafe:select}
\State {$\mathit{unsafeSet} \gets \mathit{unsafeSet} \cup \langle C_j,\mathit{imgs} \rangle$}
\EndFor

\State {\textbf{Return} $\mathit{unsafeSet}$ }

\end{algorithmic}
\caption{Algorithm for the identification of unsafe images}
\label{algo:unsafe}
\end{figure}
%\vspace{-3mm}

%\vspace{-0.2cm}
%\label{alg:executeMR}
%\end{figure}



==> algos/assignToClustersNew.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
%\begin{figure}[tb]

\begin{figure}

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
\Require (1) $R$, root cause clusters. (2) $\mathit{IS}$, set with the identifiers of the images belonging to the improvement set. (3) $\mathit{sf}$, the selection factor used in Equation~\ref{eq:U:RCC:TrS}. (4) $size_{TS}$ the size of the test set. (5) $acc_{TS}$ the accuracy for the test set. (6) $\mathit{DM}_{\mathit{IS}}$, distance matrix capturing the distance between images in the improvement set and images in \emph{TS}. 

\Ensure an associative array with the unsafe images associated to each root cause cluster
% (source inputs, follow-up inputs, output data).

%\Require $dm$, a domain model
%\Ensure $P$, a set of pairs $<Scenario, pc>$
%\State $step.visited = true$	
%\State {$\mathit{unsafeImages} \gets \mathit{empty} \mathit{List}  $}; {$\mathit{unsafeSet} \gets \mathit{empty} \mathit{Set}  $}
%\For{ y belonging to IS}
%\If{index of t < index of u}
%\State $\mathit{pairs} \mathrel{+}= 1 $
%\EndIf
%\EndFor
%\EndFor \label{algo:unsafe:distCompEnd}
\Statex
\Statex \textcolor{gray}{//Initialize the array that will contain all the images to be processed} 
\State $\mathit{rankedClustersPerImage}  \gets$ new associative array that will contain, 
\Statex\hspace{2cm}for every image, the IDs of clusters, 
\Statex\hspace{2cm}ranked based on their distance from the image

\Statex \textcolor{gray}{//Set the max number of images to be assigned to each cluster} 
\For{clusterID in R} \label{algo:unsafe:ucStart} 
\State $\mathit{Uc}[clusterID] \gets  (\mathit{size}_{TS} * \mathit{sf}) * (1-\mathit{acc}_{TS}) * \frac{\mathit{sizeOf}(R[\mathit{clusterID}])}{\mathit{sizeOf}(R)}$ \label{algo:unsafe:ucEnd}
\EndFor
\Statex \textcolor{gray}{//For each image, rank clusters, based on HeatmapDistance} 
\For{$\mathit{img}$ in $\mathit{IS}$} \label{algo:unsafe:rankStart} 
\Statex \textcolor{gray}{\hspace{2mm} //Generate an associative array capturing, for every cluster,} 
\Statex \textcolor{gray}{\hspace{2mm} the distance of $\mathit{img}$ from the closest image of the cluster}
\For{$\mathit{clusterID}$ in R} \label{algo:unsafe:rankStart:distStart}
\State $\mathit{clusterDists} \gets$ new associative array to store the distance of $\mathit{img}$
\Statex\hspace{2cm}from every cluster
\State $\mathit{closest} \gets$ use $DM_{IS}$ to identify the test set image that is  closer to $\mathit{img}$ 
\\\hspace{2cm}among the ones belonging to $\mathit{clusterID}$ 
\State $\mathit{clusterDists}[\mathit{clusterID}] \gets$ distance between $\mathit{closest}$ and $\mathit{img}$
\EndFor \label{algo:unsafe:rankStart:distEnd}
\Statex \textcolor{gray}{\hspace{4mm}//Put clusters in the correct rank for $\mathit{img}$} \label{algo:unsafe:rankStart:rankStart}
\For{rank in 1 .. $|R|$} 
\State $\mathit{clusterID} \gets$ position in $\mathit{clusterDists}$ containing the lowest value
\State $\mathit{rankedClustersPerImage}[rank][img] \gets$ 
\\\hspace{2cm}$<\mathit{clusterID},\mathit{clusterDists}[\mathit{clusterID}]>$
\State set $\mathit{clusterDists}[\mathit{clusterID}]$ to undefined
\EndFor \label{algo:unsafe:rankStart:rankEnd}
\EndFor \label{algo:unsafe:rankEnd}

\Statex \textcolor{gray}{//Assign images to clusters, trying to assign every image to the closer cluster first}
\For{rank in 1 .. $|R|$} \label{algo:unsafe:assignStart}
\State $img \gets$ the index $img$, in $\mathit{rankedClustersPerImage}[rank][img]$ \label{algo:unsafe:assign:closer}
\Statex\hspace{1.3cm}containing the lowest value, i.e., the image that is closer to any of 
\Statex\hspace{1.3cm}the clusters
\Statex \textcolor{gray}{\hspace{4mm}//Save the ID of the cluster that is closer to $\mathit{img}$} 
\State $\mathit{clusterId} \gets \mathit{rankedClustersPerImage}[rank][img]$ \label{algo:unsafe:assign:clusterId}
\State delete $\mathit{rankedClustersPerImage}[rank][img]$ \label{algo:unsafe:assign:delete}
\Statex \textcolor{gray}{\hspace{4mm}//Add the image to the cluster, if this is not already full}
\If{\textbf{sizeOf} ( $\mathit{unsafeSet}[\mathit{clusterId}]$ ) $< \mathit{Uc}[\mathit{clusterId}]$} \label{algo:unsafe:assign:full}
\State add $\mathit{img}$ to $\mathit{unsafeSet}[\mathit{clusterId}]$ \label{algo:unsafe:assign:toCluster}
\Statex \textcolor{gray}{\hspace{8mm}//Remove the image from the array with the images to process}
\State delete $\mathit{rankedClustersPerImage}[rank][img]$ for all the ranks \label{algo:unsafe:assign:delete:all}
\EndIf
\EndFor \label{algo:unsafe:assignEnd}

%
%            clusterDists[clusterID]=minimalDistance( img, clusterImages)
%
%       
%

%
%
%>         distList = getDistance(img, clusterID)
%> sortedDistList = distList.sort()
%> for order in range(len(clusters)):
%> imagesDict[order][img] = min(sortedDistList)
%>
%> assignedImages = list()
%> for order in range(len(clusters)):
%>     img = getMin(imagesDistances[order])      //finds the image with a minimal distance from any cluster
%>     clusterID = imagesDict[order][img]    //retrieve the ID of teh cluster it should be assigned to
%>     delete img from imagesDict
%>     if clustersLength[clusterID] < Uc[clusterID]:        //i.e., th emage can be assigned to the cluster
%>         clustersLength[clusterID] += 1
%>         assignedImages.append(img)         //th eimage is added to the unsafe set

%\EndFor
\State {\textbf{Return} $\mathit{unsafeSet}$ }

\end{algorithmic}
\caption{Algorithm for the identification of unsafe images}
\label{algo:unsafe}
\end{figure}
%\vspace{-3mm}

%\vspace{-0.2cm}
%\label{alg:executeMR}
%\end{figure}



==> algos/dbscan.tex <==
\begin{sloppypar}	

\begin{algorithm}[H]
	
	        \While{\textit{there is a non processed point in the dataset}}{\\
	         - Randomly select a non processed point $p$ ;\\
	         - Compute the distance between this point and all the other points in the dataset and retrieve the points within a distance $\epsilon$ ;\\
	         - If $p$ is a Core point a cluster is formed ;\\
	         - If $p$ is a Border point it will be marked as member of a cluster ;\\
	         - If $p$ is not a Border nor a Core point, it is considered Noise point ;\\
	        }
			\caption{DBSCAN}
			\label{dbscan_algorithm}
		\end{algorithm}
	\end{sloppypar}

==> notes.tex <==

\subsection{Background notes by Mohammed}
\subsection{Computer Vision}
	Computer vision is a field of artificial intelligence. It allows computers to analyze, process, and understand images. Computer vision systems are employed to extract relevant data from visual inputs to use them in other recommendation tasks.
	
	In recent years, convolutional neural networks (CNNs) have attracted much attention from the computer vision community. This success is related to different factors, such as the impressive error rate achieved by the AlexNet architecture \cite{krizhevsky2012imagenet}, the massive amounts of accessible data, and the availability of powerful graphics processing units (GPU).
	CNNs are characterized by their capacity to learn data representation compared to traditional machine learning methods. In these architectures, the feature extraction process is performed based on convolutional layers instead of using handcrafted features.
	
	To optimize the traditional CNN architecture, various structures have been proposed \cite{simonyan2014very,szegedy2015going,szegedy2016rethinking,he2016deep,howard2017mobilenets}. The main purpose was to develop deeper architectures while reducing the number of trainable parameters. VGGNet \cite{simonyan2014very} proposes the exploitation of convolutional layers associated with small receptive fields ($3 \times 3$). Inception \cite{szegedy2015going} use Inception modules instead of the standard convolutional layers \footnote{The main difference between the VGGNet and the InceptionV3 architectures is the nature of convolutional layers. VGGNet is based on the standard convolutional layers. In contrast, InceptionV3 exploit Inception blocks, where each Inception module regroups many convolutions.}. Combining these modules has successfully generated a deep network (22 layers) that reduces 12 times the number of the AlexNet's parameters \cite{krizhevsky2012imagenet}. ResNet \cite{he2016deep} introduces residual connections between convolutional layers to avoid the gradient vanishing problem. Finally, other architectures such as MobileNetV1 \cite{howard2017mobilenets} and  MobileNetV2  \cite{sandler2018mobilenetv2} have been developed for mobile and embedded vision applications.
	
	Despite their ability to learn data representation, DL networks require huge volumes of data to prevent overfitting problems. Datasets characterized by reduced volumes of data, limit the efficiency of CNNs in the classification process. As a solution, the transfer learning technique has been largely considered. This method transfers the knowledge from a generic domain, usually ImageNet, to another specific domain.
	
	\subsection{Feature extraction}
	The purpose of feature extraction is to transform unstructured data into structured raw data for their exploitation by clustering algorithms. In this study, we extracted features based on convolutional neural networks (CNNs). The standard  CNN architecture is composed of three types of layers: convolutional layers, pooling layers, and fully connected (FC) layers. 
	
	The convolutional layer is considered as the primary building block of a CNN. This layer extracts relevant features from input images during training. Besides, pooling layers are used for dimensionality reduction. Convolutional and pooling layers are stacked to form a hierarchical feature extraction module. The resulted feature map from the last pooling layer is presented as a 3D matrices of size (N, N, Nc), where N is the width and the height of the pooling layer, and Nc is its depth. For features extraction, this feature map is flattened to form a vector of size (1, $N \times N $). To resume, the CNN model receives an input image of size $(224,224,3)$. This image is then forwarded through the network's layers to generate a vector of features. The feature extraction process from all images generates a raw data represented by a 2D matrix (denoted as X), $l_i$ represent the  class categories, X and $l_i$ can be described as:  
	{
		\begin{equation}
			X = \begin{bmatrix}
				x_{11} & x_{12}  & ...  &   x_{1m} & l_2\\ 
				x_{21} &  x_{22}  & ...  & x_{2m} & l_c \\ 
				... & ...   & ...   & ...  & ... \\ 
				x_{k1} & x_{k2}  & ...  & x_{km} & l_1 \\
			\end{bmatrix}, l_i \in \left \{ l_1,l_2,...,l_{c}  \right \}, i \in [1,c] 
		\end{equation}
	}
	Where, c is the number of categories, $m = N \times N $ is the number of features, and k is the number of samples in the dataset. 
	
	In this study, we used VGG16 as a feature extraction CNN architecture. However, several CNNs architectures for feature extraction exists: InceptionV3 \cite{szegedy2015going}, VGG19 \cite{simonyan2014very}, ResNet50 \cite{ he2016deep}, and MobileNet \cite{howard2017mobilenets}. We exploited the pre-trained models on the ImageNet dataset, since, unlike the traditional feature extraction methods, CNNs must be pre-trained to perform feature extraction.  The number of extracted features is related to the used architecture, where InceptionV3, VGG16, VGG19, ResNet50, and MobileNet generated 2048, 512, 512, 2048, and 1024 features, respectively. 
	In the following sections we describe the most used CNN architectures for features extraction.
	\subsection{VGGNet}
	VGGNet \cite{simonyan2014very} is a convolutional neural network characterized by deep configurations (16 to 19 layers). The purpose of this architecture is to increase the network's depth and to minimize the number of trainable parameters.  Controlling the number of parameters helps to reduce overfitting issues. To this end,  VGGNet proposes to decrease the size of filters from $7 \times 7$ and $5 \times 5$ to $3 \times 3$. The comparative study between the number of parameters in 3 stacked convolutional layers associated with $3 \times 3$ filters and a single convolutional layer associated with $7 \times 7$   filters demonstrated that small filters reduce the total number of parameters. The number of parameters in 3 stacked convolutional layers ( $3 \times 3$ filters)  is  $3^2C^2$, on the other hand, the number of parameters in a single convolutional layer ( $7 \times 7$ filters) is $7^2C^2$, where, C is the depth of the convolutional layers. 

	To resume, VGGNet proposes to stack convolutional layers associated with small receptive fields to reduce the number of parameters and enhance non-linearity through ReLu activation functions in intermediate layers.    

	VGGNet proposes six different configurations: A, A-LRN, B, C, D, and E, where the depth varies from 11 to 19 layers. In this contribution, we exploited the configurations D and E, which are composed of 16 and 19 layers, respectively. 
	
	\subsection{InceptionV3}
	
	InceptionV3 \cite{szegedy2015going} is a refined version of Inception \cite{szegedy2016rethinking}. This network proposes other variants of Inception blocks to reduce the number of multiplications in the convolution and optimize computational complexity. These variants are based on two types of factorizations: factorization into smaller convolutions and factorization into asymmetric convolutions.  

	The standard Inception blocks use filters with a variable size ($1 \times 1$, $3 \times 3$, and $5 \times 5$)  in the same convolution instead of using a single filter's size ($3 \times 3$). The results of each filter are then stacked and considered as an input to the next convolutional layer. Using multiple filters in the same convolution helps to avoid patch alignment problems.

	The factorization into smaller convolutions proposes reducing the filter size in the standard convolutions from $5 \times 5$ to $3 \times 3$. This technique replaces $5 \times 5$ filters by two $3 \times 3$  filters to reduce the number of parameters in an Inception block by 25\%.
	
	The factorization into asymmetric convolutions propose to replace $F \times F$ convolutions by asymmetric convolutions associated with $F \times1$ and $1 \times F$ filters. This technique reduces the computational complexity by 33\% for F=3. 

	In addition to the factorization strategy, InceptionV3 exploit other techniques such as label smoothing and auxiliary classifiers.

	To resume, the InceptionV3 architecture is composed of three types of Inception blocks: A, B, C, and C that exploit different factorization techniques.
	\subsection{ResNet}
	ResNet \cite{ he2016deep} is a convolutional neural network based on residual blocks. The purpose of this architecture is to solve vanishing gradient problems in deep neural networks. During the backpropagation process, the gradient diminishes dramatically in deep networks. Small values of gradients prevent the weights from changing their values, which slow the training process. To solve this issue, ResNet introduces residual blocks. These buildings blocks present skip connections between the previous convolutional layer's input and the current convolutional layer's output. 

	ResNet proposes different configurations inspired by the VGGNet network. The depth of these configurations varies between 18 and 152 layers. We exploited the ResNet configuration with 50 layers (ResNet50) as a feature extractor in this contribution. 
	\subsection{MobileNet}
	MobileNet \cite{howard2017mobilenets} is a convolutional neural network that has been designed for mobile and embedded vision applications. This architecture is based on depthwise separable convolutions (DSC). The purpose of these buildings blocks is to reduce the number of parameters and optimize computational complexity. DSC factorize a convolution into a depthwise convolution (DC) and a pointwise convolution (PC). Unlike the standard convolutions, in DSC, a single filter is applied to each input channel. Then, the resulted channels are combined by a pointwise convolution. This process reduces the number of parameters by $\frac{1}{N} + \frac{1}{{D_k}^2}$, where $ D_k$ is the size of the filter and N is the number of filters. To construct smaller and computationally less expensive models, MobileNet introduces two hyperparameters: resolution and width multipliers. The purpose of width multiplier ($\alpha \in  \left[ 0, 1\right]$)  is to reduce the number of channels in a convolutional layer from M to $\alpha M$. Besides, the resolution multiplier reduces the computational complexity by decreasing the resolution of the input image. MobileNet is composed of 28 layers: 14 standard convolutional layers, 13 DSC, and one hidden FC. 

\subsection{Fine Tuning}
The pre-trained model on the ImageNet dataset was then used as a base model for transfer learning. Transfer learning reuses a trained model on a source task $ T_S $ on another target task $ T_T $. This technique is performed in two main steps: the network's initialization and fine-tuning. First, we initialized the new VGG16 model by the pre-trained weights P($X_s \mid Y_s$) on the ImageNet dataset instead of random initializations. We subsequently replaced the last softmax layer with a new FC layer composed of C neurons, where C is the number of labels in the target task. Finally, a subset of the first layers is frozen ($l_i \in \left\{1,...,K\right\}; K < L$), whereas, the remaining layers ($l_i \in \left\{K+1,...,L\right\}$ ; L is the number of layers) are fine-tuned on the new target task to obtain the new weights P($X_T \mid Y_T$).
\subsection{Dimensionality Reduction}
Given an instance $X_i$ which is composed of a $a$ vector of a attributes $X_i$ = $x_i^1$ , . . . , $x_i^a$ . The Dimensionality Reduction comprises the process of finding some transformation function (or map) $A$ : $\mathbb{R}^a  \rightarrow \mathbb{R}^m$, where $m < a$, to be applied on each instance $X_i$ as follows:
$Y_i$ = $A(X_i)$,
where $Y_i$ = $y_i$,...,$y_i$.


We distinguish two main different dimensionality reduction categories: (i) feature selection which consists in selecting a subset of the input features, i.e., the most relevant and non-redundant features, without operating any sort of data transformation; and (ii) feature transformation – also called feature extraction – which consists in constructing from a set of input features in high-dimensional space, a new set of features in a lower dimensional space. We used this category for our method.
\subsection{Clustering}
	Clustering is an unsupervised learning technique that divides a set of objects into clusters such that : (a) objects in the same cluster must be similar as much as possible, (b) objects in different clusters must be different as much as possible. In this work, we used DBSCAN clustering algorithm after extensive experiments on several clustering algorithms.
\subsubsection*{DBSCAN clustering Algorithm}	
DBSCAN (density-based spatial clustering of applications with noise) \cite{ester1996density} is the most used density-based clustering algorithm. It considers the points with the most neighbors as centers of the clusters (the regions with high density are considered clusters). At the same time, points with fewer neighbors are considered noise. The DBSCAN algorithm introduces two concepts of Clustering: Reachability and Connectivity.
\begin{itemize}
    \item Reachability: a point is reachable from another if the distance between them is inferior to a threshold $\epsilon$.
    \item Connectivity: if two points $p$ and $q$ are connected they belong to the same cluster. If points $p$ and $r$ are connected and $r$ and $q$ are connected, then $p$ and $q$ are also connected (transitivity). 
\end{itemize}
To apply these concepts, DBSCAN introduces two parameters: $MinPts$ and $\epsilon$.

\begin{itemize}
    \item $MinPts$: the minimum of points that a region should have to be considered dense.
    \item Threshold $ \epsilon $: a threshold to determine if a point belongs to another point's neighborhood.
\end{itemize} 
Based on the concepts described above, DBSCAN presents three types of points:
\begin{itemize}
    \item Core point:  it has at least $MinPts$ points within a distance of $\epsilon$.
    \item Border point: it is not a core point, but it belongs to at least one cluster. That means that it lies within a distance $\epsilon$ from a core point.
    \item Noise point: it's a point that is not a core point nor a border point.
\end{itemize}
Figure \eqref{dbscan} illustrates DBSCAN's point types.\\
\begin{figure}[h]
			\centerline{\includegraphics[width=0.5\textwidth]{figures/dbscan.png}}
			\caption{\label{dbscan} DBSCAN point types}
\end{figure}  
The DBSCAN algorithm proceed by taking point randomly from the dataset until all points are picked. Then for each point it determines if it's a Core, Border or Noise point based on the parameters $\epsilon$ and $MinPts$. The core point are considered centers of each cluster. The clusters are then expanded by recursively repeating the neighborhood calculation for each neighboring point.  Algorithm \eqref{dbscan_algorithm} present the DBSCAN algorithm. The main problems of DBSCAN are its sensitivity to varying density. It is also not suitable with high dimensional data.
% \begin{sloppypar}	

% \begin{algorithm}[H]
% 		\small
% 			\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
% 			\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
% 			\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% 			\Input{$\epsilon$, $MinPts$ and a set of points $N$}
% 			\Output{Clusters of points and their centers}
% 	        \While{\textit{there is a non processed point in the dataset}}{
% 	         - Randomly select a non processed point $p$ ;\\
% 	         - Compute the distance between this point and all the other points in the dataset and retrieve the points within a distance $\epsilon$ ;\\
% 	         - If $p$ is a Core point a cluster is formed ;\\
% 	         - If $p$ is a Border point it will be marked as member of a cluster ;\\
% 	         - If $p$ is not a Border nor a Core point, it is considered Noise point ;\\
% 	        }
% 			\caption{DBSCAN}
% 			\label{dbscan_algorithm}
% 		\end{algorithm}
% 	\end{sloppypar}
	
\subsection{Proposed Method}	
\subsection{Black Box Approach}
For the Black Box approach, we use a pre-trained neural network to extract a feature vector from images and cluster the images based on how similar the feature vectors are.

The pre-trained model we use is the VGG16 convolutional neural network (CNN), which is considered state-of-the-art for image recognition tasks. We use this model as a feature extractor only, meaning that we remove the final (prediction) layer to obtain a feature vector. The VGG16 architecture is illustrated in Figure \ref{vgg16}.

The first step of our approach is to preprocess the images. We downsample the images from 640x480 to 224x224 so that the dimension is compatible with that required by the pre-trained Imagenet we use for fine-tuning.

After preprocessing the images, we load the VGG16 model and remove the output layer manually. This means that the new final layer is a fully connected layer with $4096$ output neurons. This vector of $4096$ numbers is the feature vector that we use to cluster the images. After removing the final layer, we pass our preprocessed images to the network to get our feature vector through the predict function.

Since our vectors have over 4000 dimensions, it will be costly in time and memory to apply the clustering algorithm directly on that vector. We use a dimensionality reduction method (PCA) to reduce features from 4096 to 100 features.

The final step of our method is to apply the DBSCAN clustering algorithm described above on the final feature vectors. The output is a set of clusters and one cluster containing noise (outliers). 


\begin{figure}[h]
			\centerline{\includegraphics[width=0.5\textwidth]{figures/vgg16.png}}
			\caption{\label{vgg16} VGG16 architecture}
\end{figure}  

\subsection{VGG with Fine Tuning approach}
The white box approach is similar to the black box approach except that here we fine tune the top layers of the VGG16 model to fit our data. we perform the fine tuning process as follows:
\begin{itemize}
    \item Remove the fully connected nodes at the end of the network (i.e., where the actual class label predictions are made).
    \item Replace the fully connected nodes with freshly initialized ones. The number of neurons should correspond to the number of classes in our case study.
    \item Freeze earlier CONV layers earlier in the network (ensuring that any previous robust features learned by the VGG16 are not destroyed).
    \item Start training, but only train the FC layer heads.
\end{itemize}
The idea of the fine tuning is to use a black box method but train the top layers to learn from our case study.

The rest of the approach is similar to the black box method. The process of the proposed method is illustrated in Figure \ref{FE_process}.	
\begin{figure*}[h]
			\centerline{\includegraphics[width=\textwidth]{figures/FE_process.png}}
			\caption{\label{FE_process} Process of the proposed method}
\end{figure*}  	
\subsection{Experimental Results}

\begin{table}[H]
\small
\makebox[\textwidth]{

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cluster} & \textbf{Explanatory Parameters}                                                                    & \textbf{Variance Reduction}                                              & \textbf{Average Values}                                                         & \textbf{Unsafe Value}                                                & \textbf{Condition}                                                                                                                                                                                 \\ \hline
1                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}99\%\\ 98\%\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}202.51\\ 161.79\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}202.5\\ 160\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}191.25 \textless{}\textgreater 213.75\\ 145 \textless{}\textgreater 175\end{tabular}                                                                                    \\ \hline
2                & Angle                                                                                              & 99\%                                                                     & 115.41                                                                          & 112.5                                                                & 101.25 \textless{}\textgreater 123.75                                                                                                                                                              \\ \hline
3                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\\ StrangeDist\end{tabular}            & \begin{tabular}[c]{@{}c@{}}99\%\\ 98\%\\ 93\%\\ 88\%\end{tabular}        & \begin{tabular}[c]{@{}c@{}}24.36\\ 205.8\\ 17.96\\ -25\end{tabular}             & \begin{tabular}[c]{@{}c@{}}22.5\\ 220\\ 20\\ -14\end{tabular}        & \begin{tabular}[c]{@{}c@{}}11.25 \textless{}\textgreater 33.75\\ 205 \textless{}\textgreater 235\\ 10 \textless{}\textgreater 30\\ \textless -11.5\end{tabular}                                    \\ \hline
4                & Angle                                                                                              & 99\%                                                                     & 336.1                                                                           & 337.5                                                                & 191.25 \textless{}\textgreater 213.75                                                                                                                                                              \\ \hline
5                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\\ 93\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}156.66\\ 171.85\\ 15.96\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}157.5\\ 160\\ 20\end{tabular}             & \begin{tabular}[c]{@{}c@{}}146.25 \textless{}\textgreater 168.75\\ 145 \textless{}\textgreater 175\\ 10 \textless{}\textgreater 30\end{tabular}                                                    \\ \hline
6                & \begin{tabular}[c]{@{}c@{}}Angle\\ V\_Headpose\\ StrangeDist\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\\ 70\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}155.94\\ 15.53\\ -22.5\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}157.5\\ 20\\ -14\end{tabular}             & \begin{tabular}[c]{@{}c@{}}146.25 \textless{}\textgreater 168.75\\ 10 \textless{}\textgreater 30\\ \textless -11.5\end{tabular}                                                                    \\ \hline
7                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\\ StrangeDist\\ Distance\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\\ 97\%\\ 71\%\\ 96\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}204.57\\ 170.52\\ 343.19\\ -22.4\\ 21.8\end{tabular} & \begin{tabular}[c]{@{}c@{}}202.5\\ 160\\ 340\\ -14\\ 25\end{tabular} & \begin{tabular}[c]{@{}c@{}}191.25 \textless{}\textgreater 213.75\\ 145 \textless{}\textgreater 175\\ 330 \textless{}\textgreater 350\\ \textless -11.5\\ 4 \textless{}\textgreater 36\end{tabular} \\ \hline
8                & \begin{tabular}[c]{@{}c@{}}Angle\\ StrangeDist\\ Distance\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}99\%\\ 75\%\\ 95\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}246.19\\ -22.62\\ 21.87\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}247.5\\ -14\\ 25\end{tabular}             & \begin{tabular}[c]{@{}c@{}}236.25 \textless{}\textgreater 258.75\\ \textless -11.5\\ 4 \textless{}\textgreater 36\end{tabular}                                                                     \\ \hline
9                & \begin{tabular}[c]{@{}c@{}}Angle\\ V\_Headpose\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}99\%\\ 94\%\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}66.98\\ 342.13\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}67.5\\ 340\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}56.25 \textless{}\textgreater 78.75\\ 330 \textless{}\textgreater 350\end{tabular}                                                                                      \\ \hline
10               & \begin{tabular}[c]{@{}c@{}}Angle\\ V\_Headpose\\ StrangeDist\\ Distance\end{tabular}               & \begin{tabular}[c]{@{}c@{}}99\%\\ 92\%\\ 97\%\\ 97\%\end{tabular}        & \begin{tabular}[c]{@{}c@{}}246.15\\ 18.37\\ -22.8\\ 15\end{tabular}             & \begin{tabular}[c]{@{}c@{}}247.5\\ 20\\ -14\\ 25\end{tabular}        & \begin{tabular}[c]{@{}c@{}}236.25 \textless{}\textgreater 258.75\\ 10 \textless{}\textgreater 30\\ \textless -11.5\\ 4 \textless{}\textgreater 36\end{tabular}                                     \\ \hline
11               & Angle                                                                                              & 99\%                                                                     & 113.11                                                                          & 112.5                                                                & 101.25 \textless{}\textgreater 123.75                                                                                                                                                              \\ \hline
12               & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}99\%\\ 90\%\\ 99\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}247.87\\ 162.08\\ 14.67\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}247.5\\ 160\\ 20\end{tabular}             & \begin{tabular}[c]{@{}c@{}}236.25 \textless{}\textgreater 258.75\\ 145 \textless{}\textgreater 175\\ 10 \textless{}\textgreater 30\end{tabular}                                                    \\ \hline
13               & Angle                                                                                              & 99\%                                                                     & 204.48                                                                          & 202.5                                                                & 191.25 \textless{}\textgreater 213.75                                                                                                                                                              \\ \hline
\end{tabular}
}
\caption{Clusters with at least one explanatory parameter (i.e. close to an unsafe value) for GD dataset}\label{gd_rq13}
\end{table}


\begin{table}[H]
\small
\makebox[\textwidth]{

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cluster} & \textbf{Explanatory Parameters}                                             & \textbf{Variance Reduction}                                & \textbf{Average Values}                                         & \textbf{Unsafe Value}                                    & \textbf{Condition}                                                                                                           \\ \hline
1                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ H\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}84\%\\ 82\%\\ 95\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}28.27\\ -20.36\\ 173.06\end{tabular} & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 160\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 145 \textless{}\textgreater 175\end{tabular}       \\ \hline
2                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ V\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 89\%\\ 93\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}21.66\\ -16.33\\ 341.21\end{tabular} & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 340\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 330 \textless{}\textgreater 350\end{tabular}       \\ \hline
3                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ V\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}86\%\\ 82\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}26\\ -24.66\\ 343.19\end{tabular}    & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 340\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 330 \textless{}\textgreater 350\end{tabular}       \\ \hline
4                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ H\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}98\%\\ 84\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}34.75\\ -16.75\\ 207.84\end{tabular} & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 220\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 205\textless{}\textgreater{}235\end{tabular}       \\ \hline
5                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}63\%\\ 96\%\end{tabular}        & \begin{tabular}[c]{@{}c@{}}245.36\\ 171.65\end{tabular}         & \begin{tabular}[c]{@{}c@{}}247.5\\ 160\end{tabular}      & \begin{tabular}[c]{@{}c@{}}236.25\textless{}\textgreater{}258.75\\ 145 \textless{}\textgreater 175\end{tabular}              \\ \hline
6                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ Angle\end{tabular}       & \begin{tabular}[c]{@{}c@{}}98\%\\ 96\%\\ 95\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}29.5\\ -19.25\\ 208.48\end{tabular}  & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 202.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 191.25\textless{}\textgreater{}213.75\end{tabular} \\ \hline
7                & Distance                                                                    & 99\%                                                       & 35.33                                                           & 25                                                       & 4 \textless{}\textgreater 36                                                                                                 \\ \hline
\end{tabular}
}
\caption{Clusters with at least one explanatory parameter (i.e. close to an unsafe value) for OC dataset}\label{oc_rq13}
\end{table}


\begin{table}[H]
\small
\makebox[\textwidth]{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cluster} & \textbf{Explanatory Parameters}                                   & \textbf{Variance Reduction}                         & \textbf{Average Values}                                 & \textbf{Unsafe Value}                             & \textbf{Condition}                                                                                              \\ \hline
1                & Headpose\_X                                                       & 57\%                                                & -28,29                                                  & -28.88                                            & -28.88\textless{}\textgreater{}-24.16                                                                           \\ \hline
2                & Headpose\_X                                                       & 99\%                                                & 67                                                      & 74                                                & 42\textless{}\textgreater{}74                                                                                   \\ \hline
3                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}93\%\\ 95\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}11.98\\ -0.63\end{tabular}   & \begin{tabular}[c]{@{}c@{}}10\\ 0\end{tabular}    & \begin{tabular}[c]{@{}c@{}}7.5\textless{}\textgreater{}12.5\\ -2.5\textless{}\textgreater{}2.5\end{tabular}     \\ \hline
4                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 98\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-0.47\\ -0.48\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0\\ 0\end{tabular}     & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -2.5\textless{}\textgreater{}2.5\end{tabular}     \\ \hline
5                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}95\%\\ 90\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-1.8\\ -21.7\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0\\ -10\end{tabular}   & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -29.5\textless{}\textgreater{}-5.5\end{tabular}   \\ \hline
6                & Headpose\_Y                                                       & 99\%                                                & -1.63                                                   & 0                                                 & -2.5\textless{}\textgreater{}2.5                                                                                \\ \hline
7                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 92\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.53\\ -22.7\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0\\ -10\end{tabular}   & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -29.5\textless{}\textgreater{}-5.5\end{tabular}   \\ \hline
8                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-0.19\\ -2.28\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0\\ 0\end{tabular}     & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -2.5\textless{}\textgreater{}2.5\end{tabular}     \\ \hline
9                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-11.01\\ -16.61\end{tabular} & \begin{tabular}[c]{@{}c@{}}-10\\ -10\end{tabular} & \begin{tabular}[c]{@{}c@{}}-14.5\textless{}\textgreater{}-5.5\\ -29.5\textless{}\textgreater{}-5.5\end{tabular} \\ \hline
10               & Headpose\_Y                                                       & 98\%                                                & -1.67                                                   & 0                                                 & -2.5\textless{}\textgreater{}2.5                                                                                \\ \hline
\end{tabular}
}
\caption{Clusters with at least one explanatory parameter (i.e. close to an unsafe value) for HPD dataset}\label{hpd_rq13}
\end{table}


Comparison between HUDD and FE in:
\begin{itemize}
\item Percentage of clusters with at least one parameter with reduction in variance above 50\%
\item Percentage of clusters with at least one explanatory parameter

\end{itemize}

\begin{table}[H]
\small
\makebox[\textwidth]{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Case Study} & \multicolumn{2}{c|}{\textbf{HUDD}}      & \multicolumn{2}{c|}{\textbf{Feature Extraction}} \\ \hline
                    & Reduced Clusters & Explanatory Clusters & Reduced Clusters      & Explanatory Clusters     \\ \hline
GD                  & 100\%            & 86\%                 & 100\%                 & 100\%                    \\ \hline
OC                  & 57\%             & 57\%                 & 100\%                 & 100\%                    \\ \hline
HPD                 & 100\%            & 88\%                 & 100\%                 & 100\%                    \\ \hline
\end{tabular}
}
\caption{Comparison between HUDD and FE methods) for HPD dataset}\label{hudd_vs_fe}
\end{table}



==> tables/RQ1.1rt.tex <==

\GazeDNN
&100.00\%
&100.00\%
&100.00\%
&100.00\%
&100.00\%
&97.56\%
&97.56\%
&97.56\%
&97.56\%
&97.56\%
\\
\CloseDNN
&100.00\%
&100.00\%
&100.00\%
&97.30\%
&94.59\%
&94.59\%
&86.49\%
&81.08\%
&75.68\%
&56.76\%
\\


==> tables/VDA_results.tex <==
\begin{table*}[tb]
\centering

\caption{RQ2: p-values and VDA values when comparing \APPR to HUDD and the baselines}
\makebox[\textwidth]{\begin{tabular}{|C{0.7cm}|ccc|ccc|ccc|ccc|ccc|ccc|}
\hline
{\color[HTML]{000000} }        & \multicolumn{3}{c|}{{\color[HTML]{000000} GD}}                                                                                       & \multicolumn{3}{c|}{{\color[HTML]{000000} OC}}                                                                                       & \multicolumn{3}{c|}{{\color[HTML]{000000} TS}}                                                                                       & \multicolumn{3}{c|}{{\color[HTML]{000000} OD}}                                                                                     & \multicolumn{3}{c|}{{\color[HTML]{000000} HPD}}                                                                                      & \multicolumn{3}{c|}{{\color[HTML]{000000} FLD}}                                                                                 \\ \hline
{\color[HTML]{000000} }        & \multicolumn{1}{c|}{{\color[HTML]{000000} HUDD}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} BL1}}   & {\color[HTML]{000000} BL2}   & \multicolumn{1}{c|}{{\color[HTML]{000000} HUDD}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} BL1}}   & {\color[HTML]{000000} BL2}   & \multicolumn{1}{c|}{{\color[HTML]{000000} HUDD}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} BL1}}   & {\color[HTML]{000000} BL2}   & \multicolumn{1}{c|}{{\color[HTML]{000000} HUDD}} & \multicolumn{1}{c|}{{\color[HTML]{000000} BL1}}   & {\color[HTML]{000000} BL2}  & \multicolumn{1}{c|}{{\color[HTML]{000000} HUDD}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} BL1}}   & {\color[HTML]{000000} BL2}   & \multicolumn{1}{c|}{{\color[HTML]{000000} HUDD}} & \multicolumn{1}{c|}{{\color[HTML]{000000} BL1}} & {\color[HTML]{000000} BL2} \\ \hline
{\color[HTML]{000000} p-value} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.003}} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.003}} & {\color[HTML]{000000} 0.001} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.000}} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.000}} & {\color[HTML]{000000} 0.000} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.007}} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.003}} & {\color[HTML]{000000} 0.001} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.22}} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.002}} & {\color[HTML]{000000} 0.04} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.003}} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.000}} & {\color[HTML]{000000} 0.000} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.000}}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.000}}    & {\color[HTML]{000000} 0.000}    \\ \hline
{\color[HTML]{000000} VDA}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.88}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.88}}  & {\color[HTML]{000000} 0,9}   & \multicolumn{1}{c|}{{\color[HTML]{000000} 1}}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 1}}     & {\color[HTML]{000000} 1}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.85}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.96}}  & {\color[HTML]{000000} 1}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.66}} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.9}}   & {\color[HTML]{000000} 0.77} & \multicolumn{1}{c|}{{\color[HTML]{000000} 0.85}}  & \multicolumn{1}{c|}{{\color[HTML]{000000} 1}}     & {\color[HTML]{000000} 1}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 1}}     & \multicolumn{1}{c|}{{\color[HTML]{000000} 1}}    & {\color[HTML]{000000} 1}    \\ \hline
\end{tabular}}
\label{vda_results}
\end{table*}

==> tables/alexNet.tex <==
% !TEX root =  ../MAIN.tex
\begin{table}[htp]
\caption{AlexNet Layers}
\footnotesize
\begin{tabular}{|p{1cm}|p{1cm}|p{2cm}|p{1cm}|p{1cm}|}
\hline
Layer\#	& Kernel  &Type &\# Neurons &stride/pad	\\
\hline
1	&11x11 &Convolution &96 & stride 4		\\
2	&3x3 &MaxPooling &- & stride 2	\\
3	&5x5 &Convolution &256 & pad 2	\\
4	&3x3 &MaxPooling &- & stride 2	\\
5	&3x3 &Convolution &384 & pad 1	\\
6	&3x3 &Convolution &384 & pad 1	\\
7	&3x3 &Convolution &384 & pad 1	\\
8	&3x3 &MaxPooling &- & stride 2	\\
9	&- &Dense &4096 & -	\\
10	&- &Dense &4096 & -	\\
11	&- &Dense &N$^*$ & -		\\
\hline
\end{tabular}

N is the number of classes in the image classification task implemented by the DNN. It is two for \CloseDNN and eight for \GazeDNN and \FaceDNN.
\label{tab:AlexNet}
\end{table}%




%Accuracy on training set: 96% (60900/63438)
%Accuracy on test set: 96% (26100/27188)


==> tables/executinTime.tex <==
% !TEX root =  ../MAIN.tex
\begin{table}[tb]
\caption{Experiments Execution Time}
\footnotesize
\begin{tabular}{
|@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8.5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8.5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8.5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
}
\hline
\textbf{DNN}&	\textbf{Training}&	\textbf{Testing}&	\textbf{\APPR}& \textbf{\APPR} & 	\textbf{BL1}& \textbf{BL2}& \textbf{Testing} &\textbf{Total}\\
&	&	&	\textbf{Step} & \textbf{Steps}  & &	& \textbf{Improved} & \\
&	&	&	\textbf{1}& \textbf{4-7}& &	& \textbf{DNNs} & \\
\hline
\GD	& 
2.66\% &	2.00\% &	3.82\% &	26.91\% &	31.97\% &	26.64\% &	5.99\% &
375.3 \\

\CloseDNN	&
1.34\% &	8.93\% &	18.30\% &	15.63\% &	15.63\% &	13.39\% &	26.79\% &
3.7 \\

\HPD	& 
2.01\% &	2.41\% &	21.16\% &	22.93\% &	24.14\% &	20.11\% &	7.24\% &
20.7\\
\FLD &	
2.81\% &	1.41\% &	2.81\% &	28.43\% &	35.60\% &	28.10\% &	0.84\% &
177.9\\

\ODDNN	& 
2.80\% &	0.73\% &	6.83\% &	29.13\% &	30.81\% &	28.01\% &	1.68\% &
29.8\\
\TrafficDNN&	
1.89\% &	1.94\% &	29.36\% &	20.47\% &	22.63\% &	18.86\% &	4.85\% &
30.9\\
\hline
\end{tabular}


%
%



\label{tab:time}
\end{table}%




%Accuracy on training set: 96\% (60900/63438)
%Accuracy on test set: 96\% (26100/27188)


==> tables/percetageExplRCC.tex <==
\begin{table}[t]
\centering
\caption{Percentage of root cause clusters that present at least one explanatory parameter.}
\begin{tabular}{|C{3cm}|C{2cm}|C{2cm}|}
\hline
\textbf{Case Study Subject} & \textbf{SAFE} & \textbf{HUDD} \\ \hline
GD                  & \textbf{93\%}          & 86\%          \\ \hline
OC                  & \textbf{100\%}         & 57\%          \\ \hline
HPD                 & \textbf{90\%}          & 88\%          \\ \hline
\end{tabular}
\label{tab:percExplRCC}
\end{table}

==> tables/statistical_rq12.tex <==
\begin{table}[ht!]
\caption{Minimum, Maximum and Average percentage of clusters with at least one parameter showing a reduction rate above 50\% with the percentage obtained by HUDD and the p-value when comparing SAFE to HUDD.}
\begin{tabular}{|c|ccc|c|c|}
\hline
    Case Study Subjects & \multicolumn{3}{c|}{SAFE}                                         & HUDD  & p-value \\ \hline
    & \multicolumn{1}{c|}{Min}   & \multicolumn{1}{c|}{Max}   & Average &       &         \\ \hline
GD  & \multicolumn{1}{c|}{100\%} & \multicolumn{1}{c|}{100\%} & 100\%   & 100\%  & 1   \\ \hline
OC  & \multicolumn{1}{c|}{100\%} & \multicolumn{1}{c|}{100\%} & 100\%   & 57\% & 0.0005    \\ \hline
HPD & \multicolumn{1}{c|}{100\%} & \multicolumn{1}{c|}{100\%} & 100\%   & 100\% & 1    \\ \hline
\end{tabular}
\label{tab:statistical_rq12}
\end{table}

==> tables/tableRQ1.1_reduction.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[htp]
\caption{RQ1.1: Percentage of clusters showing reduction in variance}
\label{tab:RQ1.1}
\footnotesize
%the following imported .tex should be copied from IEE-2018-Ines/Experiments/Clustering/RQ1.1_scriptsR/
\begin{tabular}{p{2cm}p{7mm}p{7mm}p{7mm}p{7mm}p{7mm}p{7mm}p{7mm}p{7mm}p{7mm}p{7mm}}

Case Study& \multicolumn{4}{c}{Reduction factor} \\

& $\geqslant$ 0  &$\geqslant$ 0.20  &$\geqslant$ 0.50  &$\geqslant$ 0.90\\
%Reduction&Interval&p-value\\
\hline
\input{tables/RQ1.1rt.tex}
\hline
\end{tabular}
\end{table}%

%\begin{table}[htp]
%\caption{RQ1.1 T-test Results}
%\label{tab:RQ1.1:ttest}
%\tiny
%%the following imported .tex should be copied from IEE-2018-Ines/Experiments/Clustering/RQ1.1_scriptsR/
%\begin{subtable}{3cm}
%\center{\textbf{(a) Variance (Var)}}
%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%Reduction&Interval&p-value\\
%\hline
%\input{tables/ttestRQ1.Variance.tex}
%\hline
%\end{tabular}
%\end{subtable}
%\hspace{10mm}
%\begin{subtable}{3cm}
%\center{\textbf{(b) Mean Absolute Deviation (MeD)}}
%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%Reduction&Interval&p-value\\
%\hline
%\input{tables/ttestRQ1.MeanAD.tex}
%\hline
%\end{tabular}
%\end{subtable}
%%\hspace{10mm}
%
%\vspace{5mm}
%\begin{subtable}{3cm}
%\center{\textbf{(c) Median Absolute Deviation (MAD)}}
%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%Reduction&Interval&p-value\\
%\hline
%\input{tables/ttestRQ1.MedianAD.tex}
%\hline
%\end{tabular}
%\end{subtable}
%\hspace{10mm}
%%\begin{subtable}{3cm}
%%\center{\textbf{(d) Average of Var, MeD, MAD}}
%%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%%Reduction&Interval&p-value\\
%%\hline
%%\input{tables/ttestRQ1.measuresAVG.tex}
%%\hline
%%\end{tabular}
%%\end{subtable}
%\end{table}%




%Accuracy on training set: 96% (60900/63438)
%Accuracy on test set: 96% (26100/27188)


==> tables/tableRQ1.1_ttest.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[htp]
\caption{RQ1.1 T-test Results}
\label{tab:RQ1.1:ttest}
\footnotesize
%the following imported .tex should be copied from IEE-2018-Ines/Experiments/Clustering/RQ1.1_scriptsR/
\begin{tabular}{p{2cm}p{2cm}p{17mm}}
Reduction&Interval&p-value\\
\hline
\input{tables/ttestRQ1.Variance.tex}
\end{tabular}
\end{table}%

%\begin{table}[htp]
%\caption{RQ1.1 T-test Results}
%\label{tab:RQ1.1:ttest}
%\tiny
%%the following imported .tex should be copied from IEE-2018-Ines/Experiments/Clustering/RQ1.1_scriptsR/
%\begin{subtable}{3cm}
%\center{\textbf{(a) Variance (Var)}}
%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%Reduction&Interval&p-value\\
%\hline
%\input{tables/ttestRQ1.Variance.tex}
%\hline
%\end{tabular}
%\end{subtable}
%\hspace{10mm}
%\begin{subtable}{3cm}
%\center{\textbf{(b) Mean Absolute Deviation (MeD)}}
%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%Reduction&Interval&p-value\\
%\hline
%\input{tables/ttestRQ1.MeanAD.tex}
%\hline
%\end{tabular}
%\end{subtable}
%%\hspace{10mm}
%
%\vspace{5mm}
%\begin{subtable}{3cm}
%\center{\textbf{(c) Median Absolute Deviation (MAD)}}
%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%Reduction&Interval&p-value\\
%\hline
%\input{tables/ttestRQ1.MedianAD.tex}
%\hline
%\end{tabular}
%\end{subtable}
%\hspace{10mm}
%%\begin{subtable}{3cm}
%%\center{\textbf{(d) Average of Var, MeD, MAD}}
%%\begin{tabular}{p{1cm}p{1cm}p{7mm}}
%%Reduction&Interval&p-value\\
%%\hline
%%\input{tables/ttestRQ1.measuresAVG.tex}
%%\hline
%%\end{tabular}
%%\end{subtable}
%\end{table}%




%Accuracy on training set: 96% (60900/63438)
%Accuracy on test set: 96% (26100/27188)


==> tables/tableRQ10.tex <==
% !TEX root =  ../MAIN.tex
\begin{table*}[t!]
\footnotesize
\caption{Root cause clusters generated by \APPR.}

% \begin{tabular}{
% |@{\hspace{1pt}}p{1.2cm}
% |@{\hspace{1pt}}p{20mm}
% |p{20mm}
% |p{20mm}|
% }
% \hline
% \textbf{Case study}
% &\textbf{\# Error-inducing images}&\textbf{\# Root cause clusters}&\textbf{Ratio of inspected images}
% \\
% \hline
% \GD&5371&16&1.49\%\\
% \OC&506&14&13.82\%\\
% \HPD&1580&17&5.38\%\\
% \FLD&1554&71&22.84\%\\
% \ODDNN&838&14&8.35\%\\
% \TrafficDNN&2317&20&4.31\%\\
% \hline
% \end{tabular}\\
\centering
\makebox[0.4\textwidth]{
\begin{tabular}{|L{1.4cm}|C{0.8cm}|C{0.8cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|C{0.7cm}|}
\hline
                            & \multicolumn{2}{c|}{GD} & \multicolumn{2}{c|}{OC} & \multicolumn{2}{c|}{HPD} & \multicolumn{2}{c|}{FLD}
                            & \multicolumn{2}{c|}{OD} & \multicolumn{2}{c|}{TS}\\ \hline
                            & \APPR         & HUDD       & \APPR         & HUDD       & \APPR          & HUDD       & \APPR         & HUDD
                            & \APPR         & HUDD & \APPR         & HUDD
                            \\ \hline
                            &     & & &       &            &             &            &             &            &     &  &                  \\ \hline
\# error inducing images    & 5371       & 5371       & 506        & 506        & 1580        & 1580       & 1554       &   1554    &     838       &    838    & 2317       & 2317        \\ \hline
\# of clusters              & 23         & \textbf{16}         & 26         & \textbf{14}         & 20          & \textbf{17}         & \textbf{64}         & 71 &\textbf{ 2} & 14 & \textbf{9} & 20          \\ \hline
ratio of inspected images (\%) & 2.14       & \textbf{1.49}       & 25.69      & \textbf{13.83 }     & 6.32        & \textbf{5.38}       & \textbf{20.5}       & 22.84 & \textbf{1.19} & 8.35 & \textbf{1.94} & 4.31     \\ \hline
\end{tabular}
}
%RCC: Root Cause Clusters, IS: Improvement Set, US: Unsafe Set, BLUS: Balanced Labeled Unsafe Set, LUS: Labeled Unsafe Set, LIS: Labeled Improvement Set.
\label{table:RQ1.0:results}
\end{table*}%

%\begin{table*}[htp]
%\footnotesize
%\caption{Size of New Images Set and Retaining Set for RQ2.2}
%
%\begin{tabular}{
%|p{1cm}
%|p{1.3cm}p{7mm}p{1cm}
%|p{1.3cm}p{5mm}p{1.1cm}
%|p{1.4cm}
%||p{5mm}p{8mm}p{9mm}
%|p{5mm}p{8mm}p{9mm}}
%&\multicolumn{3}{c}{\textbf{HUDD}}&\multicolumn{3}{c}{\textbf{Baseline1}}&\multicolumn{1}{c}{\textbf{Baseline2}}&\multicolumn{3}{c}{\textbf{Accuracy Improvements}}&\multicolumn{3}{c}{\textbf{REIICC}}
%\\
%\textbf{Case study}
%&\textbf{IS}&\textbf{US}&\textbf{U}&\textbf{BLUS}
%&\textbf{US
%\\
%\hline
%\GazeDNN&17,500&12,208&16000	\\
%\CloseDNN&18,324&	\\
%\ASLDNN&21750&
%..\\
%\end{tabular}
%IS: Improvement Set, US: Unsafe Set, BLUS: Balanced Labeled Unsafe Set, BUS: Balanced Unsafe Set.
%\label{table:RQ2.2:details}
%\end{table*}%


%\begin{table*}[htp]
%\footnotesize
%\caption{Size of New Images Set and Retaining Set for RQ2.2}
%\begin{tabular}{
%|p{1cm}
%|p{1.3cm}p{7mm}p{1cm}
%|p{1.3cm}p{5mm}p{1.1cm}
%|p{1.4cm}
%||p{5mm}p{8mm}p{9mm}
%|p{5mm}p{8mm}p{9mm}}
%&\multicolumn{3}{c}{\textbf{HUDD}}&\multicolumn{3}{c}{\textbf{Baseline1}}&\multicolumn{1}{c}{\textbf{Baseline2}}&\multicolumn{3}{c}{\textbf{Accuracy Improvements}}&\multicolumn{3}{c}{\textbf{REIICC}}
%\\
%\textbf{Case study}
%&\textbf{Improvement Set}&\textbf{Unsafe Set}&\textbf{Balanced Labeled Unsafe Set}
%&\textbf{Improvement Set}&\textbf{Unsafe Set}&\textbf{Augmented Unsafe Set}
%&\textbf{Improvement Set}
%
%&\textbf{HUDD}
%&\textbf{Baseline1}
%&\textbf{Baseline2}
%
%&\textbf{HUDD}
%&\textbf{Baseline1}
%&\textbf{Baseline2}
%\\
%\hline
%\GazeDNN&17,500&	\\
%\CloseDNN&18,324&	\\
%\ASLDNN&21750&
%..\\
%\end{tabular}
%\label{table:RQ2.2:details}
%\end{table*}%




%Accuracy on training set: 96% (60900/63438)
%Accuracy on test set: 96% (26100/27188)


==> tables/tableRQ22results.tex <==
% !TEX root =  ../MAIN.tex
\begin{table}[tb]
\footnotesize
\caption{Accuracy and accuracy improvement of retrained models}

\begin{tabular}{
|@{\hspace{1pt}}p{1.2cm}
|@{\hspace{1pt}}p{10mm}p{10mm}p{10mm}
|@{\hspace{1pt}}p{10mm}p{10mm}p{10mm}
|
}
&\multicolumn{3}{c}{\textbf{p=25\%}}&\multicolumn{3}{c}{\textbf{p=100\%}}\\
\textbf{Case study}
&\textbf{HUDD}&\textbf{B1}&\textbf{B2}
&\textbf{HUDD}&\textbf{B1}&\textbf{B2}
\\
\hline
\GazeDNN&\\
\CloseDNN&\\
\ASLDNN&99.40(+5.89)&&&&\\
\TrafficDNN&&&&&\\
\end{tabular}\\
RCC: Root Cause Clusters, IS: Improvement Set, US: Unsafe Set, BLUS: Balanced Labeled Unsafe Set, LUS: Labeled Unsafe Set, LIS: Labeled Improvement Set.
\label{table:RQ2.2:details}
\end{table}%

%\begin{table*}[htp]
%\footnotesize
%\caption{Size of New Images Set and Retaining Set for RQ2.2}
%
%\begin{tabular}{
%|p{1cm}
%|p{1.3cm}p{7mm}p{1cm}
%|p{1.3cm}p{5mm}p{1.1cm}
%|p{1.4cm}
%||p{5mm}p{8mm}p{9mm}
%|p{5mm}p{8mm}p{9mm}}
%&\multicolumn{3}{c}{\textbf{HUDD}}&\multicolumn{3}{c}{\textbf{Baseline1}}&\multicolumn{1}{c}{\textbf{Baseline2}}&\multicolumn{3}{c}{\textbf{Accuracy Improvements}}&\multicolumn{3}{c}{\textbf{REIICC}}
%\\
%\textbf{Case study}
%&\textbf{IS}&\textbf{US}&\textbf{U}&\textbf{BLUS}
%&\textbf{US
%\\
%\hline
%\GazeDNN&17,500&12,208&16000	\\
%\CloseDNN&18,324&	\\
%\ASLDNN&21750&
%..\\
%\end{tabular}
%IS: Improvement Set, US: Unsafe Set, BLUS: Balanced Labeled Unsafe Set, BUS: Balanced Unsafe Set.
%\label{table:RQ2.2:details}
%\end{table*}%


%\begin{table*}[htp]
%\footnotesize
%\caption{Size of New Images Set and Retaining Set for RQ2.2}
%\begin{tabular}{
%|p{1cm}
%|p{1.3cm}p{7mm}p{1cm}
%|p{1.3cm}p{5mm}p{1.1cm}
%|p{1.4cm}
%||p{5mm}p{8mm}p{9mm}
%|p{5mm}p{8mm}p{9mm}}
%&\multicolumn{3}{c}{\textbf{HUDD}}&\multicolumn{3}{c}{\textbf{Baseline1}}&\multicolumn{1}{c}{\textbf{Baseline2}}&\multicolumn{3}{c}{\textbf{Accuracy Improvements}}&\multicolumn{3}{c}{\textbf{REIICC}}
%\\
%\textbf{Case study}
%&\textbf{Improvement Set}&\textbf{Unsafe Set}&\textbf{Balanced Labeled Unsafe Set}
%&\textbf{Improvement Set}&\textbf{Unsafe Set}&\textbf{Augmented Unsafe Set}
%&\textbf{Improvement Set}
%
%&\textbf{HUDD}
%&\textbf{Baseline1}
%&\textbf{Baseline2}
%
%&\textbf{HUDD}
%&\textbf{Baseline1}
%&\textbf{Baseline2}
%\\
%\hline
%\GazeDNN&17,500&	\\
%\CloseDNN&18,324&	\\
%\ASLDNN&21750&
%..\\
%\end{tabular}
%\label{table:RQ2.2:details}
%\end{table*}%




%Accuracy on training set: 96% (60900/63438)
%Accuracy on test set: 96% (26100/27188)


==> tables/tableRQ22setup.tex <==
% !TEX root =  ../MAIN.tex
\begin{table*}[t!]
\footnotesize
\caption{RQ2. Size of Images Set used for Retaining and Accuracy Improvement}

\begin{tabular}{
|@{\hspace{1pt}}p{7mm}@{\hspace{1pt}}
|@{\hspace{1pt}}p{4mm}p{3mm}p{6mm}
|@{\hspace{1pt}}p{5mm}@{\hspace{5pt}}p{5mm}@{\hspace{7pt}}p{6mm}
|@{\hspace{1pt}}p{5mm}@{\hspace{7pt}}p{5mm}
|p{4mm}
|p{20mm}@{\hspace{1pt}}
|@{\hspace{1pt}}p{20mm}@{\hspace{1pt}}
|@{\hspace{1pt}}p{20mm}@{\hspace{1pt}}
|p{8mm}@{\hspace{1pt}}
|p{5mm}@{\hspace{3pt}}
p{6mm}@{\hspace{1pt}}
%|@{\hspace{1pt}}p{12mm}p{13mm}p{13mm}
|
}
\hline
&\multicolumn{8}{c}{\textbf{Size of Images Sets for Retraining}}
&\multicolumn{1}{|c|}{\textbf{Accuracy}}
&\multicolumn{3}{c|}{\textbf{Accuracy (Accuracy improvement)}}
&\multicolumn{1}{c|}{\textbf{Delta}}
&\multicolumn{2}{c|}{\textbf{$\hat{A}_{12}$}}

\\
%\textbf{Case}
&\multicolumn{3}{c}{\textbf{HUDD}}
&\multicolumn{3}{c}{\textbf{B1}}&\multicolumn{2}{c|}{\textbf{B2}}
&\multicolumn{1}{|c|}{\textbf{Original}}
&\multicolumn{3}{c|}{}
&\multicolumn{1}{c|}{\textbf{wrt best}}
&\multicolumn{2}{c|}{\textbf{HUDD vs}}
\\
\textbf{DNN}
&\textbf{IS}&\textbf{US}
&\textbf{BLUS}
&\textbf{IS}&\textbf{LUS}&\textbf{ALUS}
&\textbf{IS}&\textbf{ALIS}
%&\textbf{HUDD}&\textbf{Baseline1}&\textbf{Baseline2}
&\multicolumn{1}{|c|}{\textbf{Model}}
&\textbf{HUDD}&\textbf{B1}&\textbf{B2}
&\multicolumn{1}{c|}{\textbf{Baseline}}
&\textbf{B1}&\textbf{B2}
\\
\hline
%\GazeDNN
%&W
%&16&72500&12208
%&3000
%&48000	
%%
%&12208
%&821
%&48000
%&12208
%&12208
%&95.95\%
%&96.30\% (+0.35)
%&90.25\% (-5.7)
%&94.92\% (-1.03)
%&+1.38\%
\GD
&72500
&1615
&4192	
%
&1615
&156.4
&4192
&1615
&4192
&95.95\%
&96.23\% (+0.28)
&95.77\% (-0.18)
&95.80\% (-0.15)
&+0.43\%
&0.72
&0.71
\\
\CloseDNN&
4103&
160&
336&
160&
43.4&
336&
160&
336&
88.03\%&
94.41\% (+6.38)&
91.65\% (+3.62)&
92.33\% (+4.30)&
+2.08\%&
1.00&
1.00
\\
\HPD&
4700&
481&
697&
481&
12.7&
697&
481&
697&
44.07\%&
68.13\% (+24.06)&
66.73\% (+22.66)&
66.30\% (+22.23)&
+1.40\%&
0.70&
0.72
\\
\FLD&
6864&
502&
970&
502&
34.9&
970&
502&
970&
44.99\%&
75.23\% (+30.24)&
72.02\% (+27.03)&
73.83\% (+28.84)&
+1.40\%&
0.70&
0.60
\\
%\ASLDNN
%&S
%&288
%&21750
%&1910
%&10
%&1910
%&1910
%&1910
%&1910
%&1910
%&1910
%&93.51\%
%&99.14\% (+5.63)
%&99.07\% (+5.56)
%&98.73\% (+5.22)
%&\FIXME{+0.07(0.41)}\%
%\\
\TrafficDNN
&9775
&704
&1860
&704
&53.2
&1860
&704
&1860
&81.65\%
&93.03\% (+11.38)
&92.63\% (+10.98)
&92.73\% (+11.08)
&+0.30\%
&0.83
&0.67
\\
\ODDNN
&13194
&258
&770
&258
&69.1
&770
&258
&770
&84.12\%
&97.04\% (+12.92)
&96.63\% (+12.51)
&96.67\% (+12.55)
&+0.37\%
&0.79
&0.60
\\
\hline
\end{tabular}\\
IS: Improvement Set, US: Unsafe Set, 
%U: size of root cause clusters in unsafe set; 
BLUS: Balanced Labeled Unsafe Set;
LUS: Labeled Unsafe Set (average over all the runs);
ALUS/ALIS: Augmented Labeled Unsafe/Improvement Set.
%ALIS: Augmented Labeled Improvement Set.
%*Accuracy for full test set: 96.22\%, 91.10\%, 94.95\%.
\label{table:RQ2.2:details}
\end{table*}%

%\begin{table*}[htp]
%\footnotesize
%\caption{Size of New Images Set and Retaining Set for RQ2.2}
%
%\begin{tabular}{
%|p{1cm}
%|p{1.3cm}p{7mm}p{1cm}
%|p{1.3cm}p{5mm}p{1.1cm}
%|p{1.4cm}
%||p{5mm}p{8mm}p{9mm}
%|p{5mm}p{8mm}p{9mm}}
%&\multicolumn{3}{c}{\textbf{HUDD}}&\multicolumn{3}{c}{\textbf{Baseline1}}&\multicolumn{1}{c}{\textbf{Baseline2}}&\multicolumn{3}{c}{\textbf{Accuracy Improvements}}&\multicolumn{3}{c}{\textbf{REIICC}}
%\\
%\textbf{Case study}
%&\textbf{IS}&\textbf{US}&\textbf{U}&\textbf{BLUS}
%&\textbf{US
%\\
%\hline
%\GazeDNN&17,500&12,208&16000	\\
%\CloseDNN&18,324&	\\
%\ASLDNN&21750&
%..\\
%\end{tabular}
%IS: Improvement Set, US: Unsafe Set, BLUS: Balanced Labeled Unsafe Set, BUS: Balanced Unsafe Set.
%\label{table:RQ2.2:details}
%\end{table*}%


%\begin{table*}[htp]
%\footnotesize
%\caption{Size of New Images Set and Retaining Set for RQ2.2}
%\begin{tabular}{
%|p{1cm}
%|p{1.3cm}p{7mm}p{1cm}
%|p{1.3cm}p{5mm}p{1.1cm}
%|p{1.4cm}
%||p{5mm}p{8mm}p{9mm}
%|p{5mm}p{8mm}p{9mm}}
%&\multicolumn{3}{c}{\textbf{HUDD}}&\multicolumn{3}{c}{\textbf{Baseline1}}&\multicolumn{1}{c}{\textbf{Baseline2}}&\multicolumn{3}{c}{\textbf{Accuracy Improvements}}&\multicolumn{3}{c}{\textbf{REIICC}}
%\\
%\textbf{Case study}
%&\textbf{Improvement Set}&\textbf{Unsafe Set}&\textbf{Balanced Labeled Unsafe Set}
%&\textbf{Improvement Set}&\textbf{Unsafe Set}&\textbf{Augmented Unsafe Set}
%&\textbf{Improvement Set}
%
%&\textbf{HUDD}
%&\textbf{Baseline1}
%&\textbf{Baseline2}
%
%&\textbf{HUDD}
%&\textbf{Baseline1}
%&\textbf{Baseline2}
%\\
%\hline
%\GazeDNN&17,500&	\\
%\CloseDNN&18,324&	\\
%\ASLDNN&21750&
%..\\
%\end{tabular}
%\label{table:RQ2.2:details}
%\end{table*}%




%Accuracy on training set: 96% (60900/63438)
%Accuracy on test set: 96% (26100/27188)


==> tables/ttestRQ1.MeanAD.tex <==

90\%&[ 0.62,0.78 ]&3.45e-41\\
80\%&[ 0.88,0.10 ]&9.85e-46\\
70\%&[ 1.26,0.58 ]&4.82e-43\\
60\%&[ 1.72,0.14 ]&3.79e-47\\
50\%&[ 2.27,0.76 ]&4.95e-53\\
40\%&[ 3.12,0.67 ]&1.02e-64\\
30\%&[ 4.26,0.89 ]&6.32e-78\\
20\%&[ 5.36,0.04 ]&1.69e-88\\
10\%&[ 7.05,0.70 ]&3.61e-114\\


==> tables/ttestRQ1.MedianAD.tex <==

90\%&[ 0.55,0.71 ]&1.57e-39\\
80\%&[ 0.64,0.83 ]&5.57e-38\\
70\%&[ 0.88,0.11 ]&1.19e-40\\
60\%&[ 1.17,0.47 ]&5.77e-43\\
50\%&[ 1.60,0.98 ]&1.19e-47\\
40\%&[ 2.02,0.46 ]&4.94e-52\\
30\%&[ 2.60,0.11 ]&1.94e-58\\
20\%&[ 3.63,0.21 ]&1.19e-72\\
10\%&[ 5.66,0.28 ]&4.50e-101\\


==> tables/ttestRQ1.Variance.tex <==

90\%&[ 0.84,0.05 ]&6.20e-44\\
80\%&[ 1.25,0.55 ]&2.10e-46\\
70\%&[ 1.69,0.08 ]&4.89e-49\\
60\%&[ 2.10,0.55 ]&1.75e-53\\
50\%&[ 2.55,0.05 ]&1.77e-58\\
40\%&[ 3.23,0.75 ]&5.56e-71\\
30\%&[ 3.93,0.48 ]&4.66e-81\\
20\%&[ 4.97,0.53 ]&4.24e-98\\
10\%&[ 6.45,0.97 ]&5.89e-127\\


==> tables/ttestRQ1.measuresAVG.tex <==

90\%&[ 0.59,0.75 ]&3.64e-42\\
80\%&[ 0.83,0.06 ]&1.33e-39\\
70\%&[ 1.13,0.44 ]&6.91e-40\\
60\%&[ 1.59,0.98 ]&8.36e-47\\
50\%&[ 1.98,0.43 ]&5.96e-50\\
40\%&[ 2.56,0.06 ]&2.18e-58\\
30\%&[ 3.33,0.89 ]&5.67e-68\\
20\%&[ 4.78,0.36 ]&1.59e-92\\
10\%&[ 6.61,0.19 ]&2.68e-119\\

